Quantum Bayesian networks with application to games displaying Parrondo's paradox

Bayesian networks and their accompanying graphical models are widely used for prediction and analysis across many disciplines. We will reformulate these in terms of linear maps. This reformulation will suggest a natural extension, which we will show is equivalent to standard textbook quantum mechanics. Therefore, this extension will be termed "quantum". However, the term "quantum" should not be taken to imply this extension is necessarily only of utility in situations traditionally thought of as in the domain of quantum mechanics. In principle, it may be employed in any modeling situation, say forecasting the weather or the stock market--it is up to experiment to determine if this extension is useful in practice. Even restricting to the domain of quantum mechanics, with this new formulation the advantages of Bayesian networks can be maintained for models incorporating quantum and mixed classical-quantum behavior. The use of these will be illustrated by various basic examples. Parrondo's paradox refers to the situation where two, multi-round games with a fixed winning criteria, both with probability greater than one-half for one player to win, are combined. Using a possibly biased coin to determine the rule to employ for each round, paradoxically, the previously losing player now wins the combined game with probability greater than one-half. Using the extended Bayesian networks, we will formulate and analyze classical observed, classical hidden, and quantum versions of a game that displays this paradox, finding bounds for the discrepancy from naive expectations for the occurrence of the paradox. A quantum paradox inspired by Parrondo's paradox will also be analyzed. We will prove a bound for the discrepancy from naive expectations for this paradox as well. Games involving quantum walks that achieve this bound will be presented.

==> chapter7ver2.tex <==
\chapter{Parrondo's paradox}\label{ch:parrondo}
\section{Defining the paradox}\label{sec:definingtheparadox} Suppose a two-player (or one-player versus the house) repeated game wins with probability greater than one-half for one player as does a second repeated game. Naively, it may seem that the convex combination of the two games using a (possibly biased) coin to determine which rule to employ for each round must also win for that player. However, it is possible that this combined game actually wins with probability greater than one-half for the second player. This paradoxical result is termed Parrondo's paradox~\cite{parrondo}.
\subsubsection*{Criteria for winning}\label{subsec:winning criteria} 
While this paradox is displayed for several different winning criteria (see~\cite{flitney} for instance), here the following very simple criteria will be employed for all the following games: in total, \textit{n} rounds of a game with observation set $ \mathcal{R} $ are played. Let $ \mathcal{E} $ be the $ \sigma $-algebra of observable events for each round. For a fixed set $ A\in\mathcal{E} $, if the state is in \textit{A} at the \textit{n}th round, the first player (call her Alice) wins; otherwise, the second player (call him Bob) wins--regardless of what was observed at the preceding rounds. (For one traditional formulation of Parrondo's paradox, $ \mathcal{X}=\mathbb{Z} $, $ \mathcal{E} $ is its power set, and $ A=\mathbb{Z}^{+} $.~\cite{parrondo}) It is easy to see the applicability of this criterion for many different real-life situations--for instance, the difference of scores in sports games or stock options in finance.
\section{Classical observed Markov chain game}\label{sec:classicalobservable}
\subsection{Defining the game}
Following the traditional method for Bayesian networks, the graphical model for the Markov chain game is:
\begin{align}\label{fig:classicgame}
\setlength{\unitlength}{.85 in}
\begin{picture}(5.5,.5)
\put(1,.1){\circle{.2}}
\put(2,.1){\circle{.2}}
\put(3,.1){\circle{.2}}
\put(1,.25){1}
\put(2,.25){2}
\put(3,.25){3}
\put(1.08,.1){\vector(1,0){.82}}
\put(2.08,.1){\vector(1,0){.82}}
\put(3.08,.1){\vector(1,0){.82}}
\put(4,.1){$\cdots$}
\put(4.3,.1){$\cdots$}
\put(4.5,.1){\vector(1,0){.4}}
\put(5,.1){\circle{.2}}
\put(5,.25){\textit{n}}
\put(4.9,.1){\line(1,0){.19}}
\put(5,.009){\line(0,1){.185}}
\end{picture}
\end{align}
Let $ \mu $ be the initial marginal probability measure. For the subsequent nodes, take all the transition probability functions to be the same $ \tau(\cdot\vert\cdot) $. The joint probability to observe outcomes $ (x_{1},x_{2},\ldots,x_{n})\in A_{1}\times A_{2}\times\cdots\times A_{n} $, for any $ A_{1}, A_{2},\ldots, A_{n}\in\mathcal{E} $, is then
\begin{equation}
(R_{A_{n}}\circ L\circ\cdots\circ R_{A_{2}}\circ L\circ R_{A_{1}}\mu)(\mathcal{X})
\end{equation}
for \textit{L} the map induced by $  \tau(\cdot\vert\cdot) $ (see \ref{eq:transitioninducedmap}) and $ R_{A} $ the restriction map (see \S\ref{sec:copymap}).
Then the probability to observe the system has state in \textit{A} at the $ n $th round (so Alice wins), denoted $ P_{A,n} $, is given by
\begin{equation}\label{eq:matrixproduct}
(R_{A}\circ \underbrace{L\circ\cdots\circ L}_{n-1}\mu)(\mathcal{X})
\end{equation}
In the common case where the events $ \mathcal{E} $ are generated by a finite number of sets, the transition probability functions are stochastic transition matrices, the initial measure is a stochastic column vector, and the maps are given by having the matrices act on the vector in the usual matrix product. 
\subsubsection*{Combining two games}
Now suppose we have a second game with the same structure, but a different transition probability function for each round, $ \tau'(\cdot\vert\cdot) $ (there can also be a different initial marginal probability, but that will be of no consequence for the limit we will take). The probability to observe the system has its state in \textit{A} at the $ n $th round is denoted $ P'_{A,n} $. The two games can be combined by flipping a (possibly biased) coin at each round, playing according to the first game if the coin is heads, which occurs with probability $ p $, and according to the second if the coin is tails, which occurs with probability $ 1-p $. The graphical model for the combined game is:
\begin{align}\label{subsec:classicgamecombined}
\setlength{\unitlength}{.85 in}
\begin{picture}(5.2,1.3)
\put(1,.1){\circle{.2}}
\put(2,.1){\circle{.2}}
\put(3,.1){\circle{.2}}
\put(1,.25){1}
\put(2,.25){2}
\put(3,.25){3}
\put(1.09,.1){\vector(1,0){.8}}
\put(2.09,.1){\vector(1,0){.8}}
\put(3.09,.1){\vector(1,0){.8}}
\put(4,.1){$\cdots$}
\put(4.3,.1){$\cdots$}
\put(4.5,.1){\vector(1,0){.4}}
\put(5,.1){\circle{.2}}
\put(5,.25){\textit{n}}
\put(4.9,.1){\line(1,0){.19}}
\put(5,.009){\line(0,1){.185}}
\put(1.75,.8){\circle{.2}}
\put(2.75,.8){\circle{.2}}
\put(4.75,.8){\circle{.2}}
\put(1.78,.72){\vector(1,-3){.18}}
\put(2.78,.72){\vector(1,-3){.18}}
\put(4.78,.72){\vector(1,-3){.18}}
\put(1.4,1){heads,tails}
\put(2.4,1){heads,tails}
\put(4.4,1){heads,tails}
\end{picture}
\end{align}

For the combined game, the transition probability function for each round is
\begin{equation}
\tau(\cdot\vert\cdot,c)=\begin{cases}\tau(\cdot\vert\cdot)&\text{ if }c=\text{heads}\\\tau'(\cdot\vert\cdot)&\text{ if }c=\text{tails}\end{cases}
\end{equation} 
Let $ M_{c} $ be the map induced by $  \tau(\cdot\vert\cdot,c) $. The marginal probability to then observe the system is in $ A $ for the $ n $th round, denoted $ P_{A,n}^{\text{comb}} $, is then
\begin{equation}\label{eq:matrixproduct2}
\sum_{\begin{scriptsize}c_{2}\in\left\lbrace \!\!\begin{array}{l}\text{heads}\\\text{tails}\end{array}\!\!\right\rbrace\end{scriptsize}}\!\!\!\cdots\!\!\!\sum_{\begin{scriptsize}c_{n}\in\left\lbrace \!\!\begin{array}{l}\text{heads}\\\text{tails}\end{array}\!\!\right\rbrace\end{scriptsize}}\!\!\!\left( \prod_{k=1}^{n}\text{Prob}(c_{k})\right)(R_{A}\circ M_{c_{n}}\circ\cdots\circ M_{c_{2}}\mu)(\mathcal{X})=(R_{A}\circ \underbrace{L''\circ\cdots\circ L''}_{n-1}\mu)(\mathcal{X})
\end{equation}
for $ L'' $ the map induced by $ \tau''(\cdot\vert\cdot)=p\,\tau(\cdot\vert\cdot)+(1-p)\tau'(\cdot\vert\cdot) $. Note that we have a convex combination of maps, $ L''=pL+(1-p)L' $.
\subsection{Bounds on the extent of the paradox}
Let \textit{p} be the probability for the coin to give heads. Then, for $ p\in(0,1) $, one may expect the probability for Alice to win the combined game would necessarily be between the probabilities for the individual games, with 
\begin{equation}\label{naiveexpectation}
\min\lbrace P_{A,n}, P'_{A,n}\rbrace< P_{A,n}^{\text{comb}}<\max\lbrace P_{A,n}, P'_{A,n}\rbrace
\end{equation}
if $ P_{A,n}\neq P'_{A,n} $ and $  P_{A,n}^{\text{comb}}=P_{A,n}= P'_{A,n} $ if $ P_{A,n}= P'_{A,n} $. Parrondo's paradox is that not only is that expectation false, but it is possible for Alice to have probability greater than one-half of winning each of the individual games, yet less than one-half for the combined game.

In the common case where the events $ \mathcal{E} $ are generated by a finite number of sets, the Perron-Frobenius theorem~\cite{seneta}~\cite{norrisPF} gives the conditions on \textit{L} for there to be a stochastic vector $ \nu $, termed the Perron-Frobenius eigenvector\footnote{Also termed the \textit{invariant probability distribution}~\cite{feller}, the \textit{steady-state probability vector}~\cite{martin}, or the \textit{invariant measure}~\cite{norris} in the literature.}, such that the sequence $ \langle L^{j}\nu_{0}\rangle $ converges in norm to $ \nu $ regardless of the initial stochastic vector $ \nu_{0} $. By generalization, we introduce the following definition:
\paragraph*{Definition 7.2.1} A linear map \textit{L} from $ \mathcal{F} $-measures on $ \mathcal{X} $ to $ \mathcal{F} $-measures on a set $ \mathcal{X} $ has the \textit{Perron-Frobenius property}, $ \mathcal{PF}(\mathcal{X},\mathcal{E}) $, if there is a measure $ \nu $, termed the \textit{Perron-Frobenius eigenvector}, such that the sequence $ \langle L^{j}\nu_{0}\rangle $ converges in total-variation norm to $ \nu $ regardless of the initial unit-norm measure $ \nu_{0} $.
\medskip\\
Now assume the transition probability functions $ \tau $ and $ \tau' $ are such that induced maps \textit{L} and \textit{L}$ ' $ each are in $\mathcal{PF}(\mathcal{X};\mathcal{E})$, as well is their convex combination, $ pL+(1-p)L' $. Then let $ P_{A}$, $ P'_{A} $, and $ P_{A}^{\text{comb}} $ be the limits as $ n\to \infty $ of $ P_{A,n} $, $ P'_{A,n}$ and $ P_{A,n}^{\text{comb}} $ respectively. We then have the question of what values of $\left(P_{A},P'_{A},P_{A}^{\text{comb}}\right)\in[0,1]^{\times 3} $ occur. 
\paragraph*{Definition 7.2.2} The \textit{classically allowed region}, denoted $ \mathcal{C}(A,\mathcal{X},\mathcal{E},p) $, is the set of all $\left(P_{A},P'_{A},P_{A}^{\text{comb}}\right)\in[0,1]^{\times 3} $ that occur, for fixed \textit{A}, $ \mathcal{X}$, $ \mathcal{E}$, and $ p $, over all possible transition probability functions $ \tau $ and $ \tau' $. 
\medskip\\
The existence of the paradox is then determined by the intersection of $ \mathcal{C} $ with the cube $ \left(\frac{1}{2},1\right]\times\left(\frac{1}{2},1\right]\times\left[0,\frac{1}{2}\right) $. For $ p=1 $, $ P_{A}^{\text{comb}}=P_{A} $ and for $ p=0 $, $ P_{A}^{\text{comb}}=P'_{A} $; clearly no paradox is possible. We have the following theorems for $ p\in(0,1) $, which indicate that there are basically only two possibilities, depending on whether we have effectively a two-state system or one with more than two states, as determined by the event $ \sigma $-algebra $ \mathcal{E} $.  
\paragraph*{Theorem 7.2.3} For $ p\in(0,1) $, if there are nonempty, disjoint subsets $ A,B,C\in \mathcal{E} $ with $  A\cup B\cup C=\mathcal{X} $, then $ \mathcal{C}\supset(0,1)^{\times 3} $.
\paragraph*{Proof} Fix any $ P_{A},P'_{A}\in(0,1) $. Then take any $ \varepsilon>0 $ sufficiently small such that both the matrices
\begin{align}
\mathbf{T}&=\left[\begin{array}{ccc}1-(1-s)\varepsilon-\left(\frac{1}{P_{A}}-1-\varepsilon\right)\varepsilon^{2}&\varepsilon^{2}&1-s\\\left(\frac{1}{P_{A}}-1-\varepsilon\right)\varepsilon^{2}&1-\frac{P_{A}s\varepsilon}{1-(1+\varepsilon)P_{A}}-\varepsilon^{2}&s\\(1-s)\varepsilon&\frac{P_{A}s\varepsilon}{1-(1+\varepsilon)P_{A}}&0\end{array}\right]\\
\mathbf{T}'&=\left[\begin{array}{ccc}1-\frac{1-P'_{A}}{P'_{A}}\varepsilon^{2}&\varepsilon^{2}&\frac{1}{2}\\\frac{1-P'_{A}}{P'_{A}}\varepsilon^{2}&1-\varepsilon^{2}&\frac{1}{2}\\0&0&0\end{array}\right]\nonumber
\end{align}
are stochastic matrices for all values of $ s\in[0,1] $. Take the transition probability functions to be
\begin{align}
\left[\begin{array}{ccc}\tau(A\vert x\in A)&\tau(A\vert x\in B)&\tau(A\vert x\in C)\\\tau(B\vert x\in A)&\tau(B\vert x\in  B)&\tau(B\vert x\in C)\\\tau(C\vert x\in A)&\tau(C\vert x\in B)&\tau(C\vert x\in C)\end{array} \right]&=\mathbf{T}\\
\left[\begin{array}{ccc}\tau'(A\vert x\in A)&\tau'(A\vert x\in B)&\tau'(A\vert x\in C)\\\tau'(B\vert x\in A)&\tau'(B\vert x\in B)&\tau'(B\vert x\in C)\\\tau'(C\vert x\in A)&\tau'(C\vert x\in B)&\tau'(C\vert x\in C)\end{array} \right]&=\mathbf{T}'\nonumber
\end{align}
Then the required calculations reduce to matrix products. Since the maps are assumed to have the Perron-Frobenius property, the initial probabilities chosen for \textit{A}, \textit{B}, and \textit{C} are irrelevant. 

By the deliberate construction of \textbf{T} and \textbf{T}$ ' $, the first entry of the Perron-Frobenius eigenvector of \textbf{T} is indeed $ P_{A} $ for every $ s\in[0,1] $ and the first entry of the Perron-Frobenius eigenvector of \textbf{T}$ ' $ is indeed $ P'_{A} $. The first entry of the Perron-Frobenius eigenvector of $ p\mathbf{T}+(1-p)\mathbf{T}' $, which gives $ P_{A}^{\text{comb}} $, varies continuously\footnote{The eigenvectors of a matrix are continuous functions of the entries of the matrix in any open set where the eigenvalues are distinct.} from
\begin{equation}
\dfrac{\varepsilon}{\frac{p(1-p)}{2}+\varepsilon\left(\frac{p}{P_{A}}+\frac{1-p}{P'_{A}}\right)}=\mathcal{O}(\varepsilon)
\end{equation}
to
\begin{equation}
\dfrac{1}{1+\dfrac{2\varepsilon\left(\frac{1}{P_{A}}-1-\varepsilon+\varepsilon p\right)\left(\frac{p}{P_{A}}+\frac{1-p}{P'_{A}}-1-\varepsilon p\right)}{p(1-p)+2\varepsilon\left(\frac{1}{P_{A}}-1-\varepsilon\right)}}=1-\mathcal{O}(\varepsilon)
\end{equation}
as $ s $ goes from zero to one. Since $ \varepsilon $ may be taken arbitrarily small, every value for $ P_{A}^{\text{comb}}\in (0,1) $ is in the allowed region for the fixed values of $ P_{A} $ and $ P'_{A} $. $ \square $
\paragraph*{Theorem 7.2.4} If $ \mathcal{E}=\lbrace\varnothing, A,\tilde{A},\mathcal{X}\rbrace $, then $ \mathcal{C} $ is given by (\ref{naiveexpectation}), so the paradox cannot occur.
\paragraph*{Proof} Define the stochastic matrix \textbf{S} by 
\begin{equation}
\mathbf{S}=\left[\begin{array}{ll}\tau(A\,\vert\,x\in A)&\hspace{.1 in}\tau(A\,\vert\, x\in\tilde{A})\\\tau(\tilde{A}\,\vert\, x\in A)&\hspace{.1 in}\tau(\tilde{A}\,\vert\, x\in\tilde{A})\end{array} \right] 
\end{equation}
and the stochastic matrix $ \mathbf{S}' $ by 
\begin{equation}
\mathbf{S}'=\left[\begin{array}{ll}\tau'(A\,\vert\,x\in A)&\hspace{.1 in}\tau'(A\,\vert x\in\tilde{A})\\\tau'(\tilde{A}\,\vert\,x\in A)&\hspace{.1 in}\tau'(\tilde{A}\,\vert\,x\in\tilde{A})\end{array} \right] 
\end{equation}
For fixed $ P_{A}, P'_{A}\in (0,1] $, express \textbf{S} and \textbf{S}$'$ as
\begin{equation}
\mathbf{S}=\left[\begin{array}{cc}1-\left(\frac{1}{P_{A}}-1\right)\zeta&\zeta\\\left(\frac{1}{P_{A}}-1\right)\zeta&1-\zeta\end{array} \right],\mathbf{S}'=\left[\begin{array}{cc}1-\left(\frac{1}{P'_{A}}-1\right)\xi&\xi\\\left(\frac{1}{P'_{A}}-1\right)\xi&1-\xi\end{array} \right] 
\end{equation} 
for $ \zeta\in\left(0,\min\lbrace \frac{P_{A}}{1-P_{A}},1\rbrace\right] $ and $ \xi\in\left(0,\min\lbrace \frac{P'_{A}}{1-P'_{A}},1\rbrace\right] $. By the deliberate construction of \textbf{S} and \textbf{S}$ ' $, the first entry of the Perron-Frobenius eigenvector of \textbf{S} is indeed $ P_{A} $ for every $ \zeta $ and the first entry of the Perron-Frobenius eigenvector of \textbf{S}$ ' $ is indeed $ P'_{A} $ for every $ \xi $. For $ P_{A}\neq P'_{A} $, the first entry of the Perron-Frobenius eigenvector of $ p\mathbf{S}+(1-p)\mathbf{S}' $, which gives $ P_{A}^{\text{comb}} $, varies continuously in the interval $ \left(\min\lbrace P_{A}, P'_{A}\rbrace,\max\lbrace P_{A}, P'_{A}\rbrace\right) $ as $ \zeta,\xi $ vary over their allowed values, approaching the extreme values only as either $ \zeta $ or $ \xi $ go to zero since it is a linear rational function in $ \zeta $ and $ \xi $. For $ P_{A}=P'_{A} $, $ P_{A}^{\text{comb}} $ shares this common value for all $ \zeta,\xi $. 

For $ P_{A}=0$, $ P'_{A}\in (0,1] $, express \textbf{S} as $ \left[\begin{array}{cc}1-\zeta&0\\\zeta&1\end{array} \right] $ for $ \zeta\in(0,1] $ and \textbf{S}$'$ as above. Then the first entry of the Perron-Frobenius eigenvector of \textbf{S} is $ P_{A}=0 $ for every $ \zeta $. The first entry of the Perron-Frobenius eigenvector of $ p\mathbf{S}+(1-p)\mathbf{S}' $, which gives $ P_{A}^{\text{comb}} $, varies continuously in the interval $ \left(0,P'_{A}\right) $ as $ \zeta,\xi $ vary over their allowed values, approaching the bounds as either $ \zeta $ or $ \xi $ go to zero. The symmetric situation holds for $ P'_{A}=0$, $ P_{A}\in (0,1] $. Finally, for $ P_{A} =P'_{A}=0 $, express \textbf{S} as $ \left[\begin{array}{cc}1-\zeta&0\\\zeta&1\end{array} \right] $ for $ \zeta\in(0,1] $ and \textbf{S}$'$ as $\left[\begin{array}{cc}1-\xi&0\\\xi&1\end{array} \right] $ for $ \xi\in(0,1] $. Then $ P_{A}^{\text{comb}}=0 $ for all $ \zeta,\xi $. $ \square $ 
\subsection{Understanding the cause of the paradox}\label{subsec:understandingtheparadox}
While surprising when approached from the game context, mathematically the cause of the paradox is straightforward: the coefficients of the Perron-Frobenius eigenvector of a convex combination of two matrices, $ M_{1},M_{2}\to tM_{1}+(1-t)M_{2} $, need not be in the convex hull of the coefficients of the Perron-Frobenius eigenvectors of each matrix. Large discrepancies are possible for certain slivers of parameter values near where eigenvalues coalesce and the resulting eigenvectors are discontinuous functions of the parameters.  

A similar cause is at play in the following analogous hidden classic and quantum versions of the preceding game. In each case, there is a convex space of matrices of spectral radius one determining the behavior of the system. A coin flip determining the rule to employ for the next round has the effect of forming a convex combination of the matrices for each rule. In the limit as the number of rounds goes to infinity, only the eigenvector of the matrix with eigenvalue one is of importance, but the coefficients for this eigenvector are not in the convex hull of the coefficients of the eigenvectors of each matrix, leading to the paradox.
\section{Classical hidden-Markov chain game}\label{sec:classicalhidden}
\subsection{Defining the combined game}
As will be proved below, it is possible to have Parrondo's paradox with a game for a system with two states if the system is hidden. The game arises from a generalization of the of the commonly utilized hidden-Markov model~\cite{jensenhm} to include imagined back-reaction on the hypothesized hidden state. The standard graphical model (with hidden nodes in gray) is:
\begin{align}
\definecolor{gray}{gray}{0.5}
\setlength{\unitlength}{.8 in}
\begin{picture}(5.8,1.3)
\color{gray}{\put(.5,.1){\circle{.2}}}
\put(1.5,.1){\circle{.2}}
\put(2.5,.1){\circle{.2}}
\put(3.5,.1){\circle{.2}}
\put(5,.1){\circle{.2}}
\put(.595,.1){\vector(1,0){.8}}
\put(1.595,.1){\vector(1,0){.8}}
\put(2.595,.1){\vector(1,0){.8}}
\put(3.595,.1){\vector(1,0){.4}}
\put(4,.1){$\cdots$}
\put(4.3,.1){$\cdots$}
\put(4.5,.1){\vector(1,0){.4}}
\put(.585,.143){\vector(2,3){.375}}
\put(1.585,.143){\vector(2,3){.375}}
\put(2.585,.143){\vector(2,3){.375}}
\put(3.585,.143){\line(2,3){.3}}
\put(5.085,.143){\vector(2,3){.375}}
\color{black}{\put(1,.8){\circle{.2}}}
\put(2,.8){\circle{.2}}
\put(3,.8){\circle{.2}}
\put(5.5,.8){\circle{.2}}
\put(1,.95){1}
\put(2,.95){2}
\put(3,.95){3}
\put(5.5,.95){\textit{n}}
\put(.9,.8){\line(1,0){.19}}
\put(1,.709){\line(0,1){.185}}
\put(1.9,.8){\line(1,0){.19}}
\put(2,.709){\line(0,1){.185}}
\put(2.9,.8){\line(1,0){.19}}
\put(3,.709){\line(0,1){.185}}
\put(5.4,.8){\line(1,0){.19}}
\put(5.5,.709){\line(0,1){.185}}
\put(1.085,.757){\vector(2,-3){.375}}
\put(2.085,.757){\vector(2,-3){.375}}
\put(3.085,.757){\vector(2,-3){.375}}
\end{picture}
\end{align}
However, as has been mentioned in \S\ref{sec:transition}, this requires interpreting probabilities and/or conditional probabilities concerning unobservable events, which are meaningless in both Bayesian and frequentist interpretations of probability. Also, this approach has no analogy in the quantum case.

Therefore, following the program we have laid out in the first part of this dissertation, the information for hidden nodes can simply be regarded as linear maps on measures, which is preferable in both avoiding metaphysical notions and in having analogous meaning in the quantum case. (As has been mentioned in \S\ref{sec:transition}, this may allow additional maps which do not arise from transition probability functions, but these are not of great interest and are not an important motivation for making the change.) Using the pince-nez construction (see \S\ref{sec:constructs}), this becomes: 
\begin{align}\label{fig:hiddengame}
\setlength{\unitlength}{.8 in}
\begin{picture}(5.5,.8)
\color{red}
\put(.1,.1){\oval(.2,.2)[r]}
\put(0,.2){\line(1,0){.1}}
\put(0,0){\line(1,0){.1}}
\put(0,0){\line(0,1){.2}}
\put(1,.1){\circle{.2}}
\put(2,.1){\circle{.2}}
\put(3.5,.1){\circle{.2}}
\put(4.5,.1){\circle{.2}}
\put(5.5,.1){\oval(.2,.2)[l]}
\put(5.5,.2){\line(1,0){.1}}
\put(5.5,0){\line(1,0){.1}}
\put(5.6,0){\line(0,1){.2}}
\put(.2,.1){\vector(1,0){.7}}
\put(1.09,.1){\vector(1,0){.8}}
\put(2.09,.1){\line(1,0){.5}}
\put(2.7,.05){$\cdots$}
\put(2.89,.1){\vector(1,0){.5}}
\put(3.59,.1){\vector(1,0){.8}}
\put(4.59,.1){\vector(1,0){.8}}
\put(.89,.1){\line(0,1){.1}}
\put(1.89,.1){\line(0,1){.1}}
\put(3.39,.1){\line(0,1){.1}}
\put(4.39,.1){\line(0,1){.1}}
\color{black}
\put(1,.3){\circle{.2}}
\put(2,.3){\circle{.2}}
\put(3.5,.3){\circle{.2}}
\put(4.5,.3){\circle{.2}}
\put(1,.45){1}
\put(2,.45){2}
\put(3.5,.45){$ n-1 $}
\put(4.5,.45){\textit{n}}
\put(4.4,.3){\line(1,0){.19}}
\put(4.5,.209){\line(0,1){.185}}
\put(.89,.2){\line(0,1){.1}}
\put(1.89,.2){\line(0,1){.1}}
\put(3.39,.2){\line(0,1){.1}}
\put(4.39,.2){\line(0,1){.1}}
\end{picture}
\end{align}
Employing option \textbf{I'} (the results can be readily recast for option \textbf{II} or more general forms of option \textbf{I}--see \S\ref{sec:optionIandII}), we have the following definition:
\paragraph*{Definition 7.3.1} A \textit{hidden-Markov-with-back-reaction-model} ($ \mathcal{R} $, $ \tau $, $ \mathcal{H} $, $ \mu $, \textit{L}, $ \nu_{0} $) is composed of: an observation set $ \mathcal{R} $ with base measure $\eta $, a hidden set $ \mathcal{H} $ with base measure $\mu $, a pince-nez map $ L\in\mathcal{B}\left(L^{1}(\mathcal{H};\mu),L^{1}(\mathcal{R}\times\mathcal{H};\eta\times\mu)\right) $, and an initial, unit-norm measure $\nu_{0}$ on $ \mathcal{H} $ that is absolutely continuous with respect to $ \mu  $.
\medskip\\
Then the joint probability to observe $ (x_{1},x_{2},\ldots,x_{n})\in A_{1}\times A_{2}\times\cdots\times A_{n} $, for any $ \eta $-measurable $ A_{1}, A_{2},\ldots, A_{n} $, is 
\begin{equation}\label{eq:jointclasicalhiddenchain}
\int_{\mathcal{H}}\left(S_{A_{n}}\circ L\circ\cdots\circ S_{A_{1}}\circ L\frac{d\nu_{0}}{d\mu}\right) d\mu
\end{equation}
for $ S_{A} $ the linear map from $ L^{1}(\mathcal{R}\times\mathcal{H};\eta\times\mu) $ to $ L^{1}(\mathcal{H};\mu) $ given by the partial integration $ S_{A}f=\int_{A}f\,d\eta $. Employing this model for the game, then the marginal probability for the observation to be in \textit{A} at the $ n $th round (so Alice wins) is 
\begin{equation}\label{eq:probwinningclassicalhidden}
P_{A,n}=\int_{\mathcal{H}}\left(S_{A}\circ L\circ \underbrace{N\circ\cdots\circ N}_{n-1}\frac{d\nu_{0}}{d\mu}\right) \;d\mu
\end{equation}
where $ N\in\mathcal{B}\left(L^{1}(\mathcal{H};\mu)\right)  $ is defined as the map $ N=S_{\mathcal{R}}\circ L $. Because of the definition of the game, it is possible to reduce to the case where the event space for $ \mathcal{R} $ is simply $ \mathcal{E}=\lbrace\varnothing, A,\tilde{A},\mathcal{X}\rbrace $ and its base measure $ \eta $ is the measure with $ \eta(A)=\eta(\tilde{A})=1 $.

Now suppose there is a second model with the same data except for a different pince-nez $ L' $ for each round (it is also possible to have a different initial measure, but since the limit as $ n\to\infty $ will be taken, this is of no consequence). Once again, the two models can be combined by flipping a (possibly biased) coin at each round. The graphical model is:
\begin{align}\label{fig:combinedhiddengame}
\setlength{\unitlength}{.8 in}
\begin{picture}(5.5,1.3)
\color{red}
\put(.1,.1){\oval(.2,.2)[r]}
\put(0,.2){\line(1,0){.1}}
\put(0,0){\line(1,0){.1}}
\put(0,0){\line(0,1){.2}}
\put(1,.1){\circle{.2}}
\put(2,.1){\circle{.2}}
\put(3.5,.1){\circle{.2}}
\put(4.5,.1){\circle{.2}}
\put(5.5,.1){\oval(.2,.2)[l]}
\put(5.5,.2){\line(1,0){.1}}
\put(5.5,0){\line(1,0){.1}}
\put(5.6,0){\line(0,1){.2}}
\put(.2,.1){\vector(1,0){.7}}
\put(1.09,.1){\vector(1,0){.8}}
\put(2.09,.1){\line(1,0){.5}}
\put(2.89,.1){\vector(1,0){.5}}
\put(2.7,.05){$\cdots$}
\put(3.59,.1){\vector(1,0){.8}}
\put(4.59,.1){\vector(1,0){.8}}
\put(.89,.1){\line(0,1){.1}}
\put(1.89,.1){\line(0,1){.1}}
\put(3.39,.1){\line(0,1){.1}}
\put(4.39,.1){\line(0,1){.1}}
\color{black}
\put(1,.3){\circle{.2}}
\put(2,.3){\circle{.2}}
\put(3.5,.3){\circle{.2}}
\put(4.5,.3){\circle{.2}}
\put(1,.45){1}
\put(2,.45){2}
\put(3.5,.45){$ n-1 $}
\put(4.5,.45){\textit{n}}
\put(4.4,.3){\line(1,0){.19}}
\put(4.5,.209){\line(0,1){.185}}
\put(.89,.2){\line(0,1){.1}}
\put(1.89,.2){\line(0,1){.1}}
\put(3.39,.2){\line(0,1){.1}}
\put(4.39,.2){\line(0,1){.1}}
\put(.75,.8){\circle{.2}}
\put(1.75,.8){\circle{.2}}
\put(3.25,.8){\circle{.2}}
\put(4.25,.8){\circle{.2}}
\put(.78,.72){\vector(1,-4){.11}}
\put(1.78,.72){\vector(1,-4){.11}}
\put(3.28,.72){\vector(1,-4){.11}}
\put(4.28,.72){\vector(1,-4){.11}}
\put(.3,1){\{heads,tails\}}
\put(1.5,1){\{heads,tails\}}
\put(2.8,1){\{heads,tails\}}
\put(4,1){\{heads,tails\}}
\end{picture}
\end{align}
Let $ \gamma $ be the previously given probability measure for the coin of \textit{p} for heads and $ 1-p $ for tails, with base measure the counting measure. For simplicity of notation, we will identify $ \gamma $ with its Radon-Nikod\'{y}m derivative $ \frac{d\gamma}{d\text{count}} $. For the combined game, the map for each round is
\begin{equation}
M(f\otimes \gamma)=p\,Lf+(1-p)L'f=L''f
\end{equation}  
for $ L''=p\,L+(1-p)L' $. Let $ N',N''\in\mathcal{B}\left(L^{1}(\mathcal{H};\mu)\right) $ be defined using $ L',L''$ as \textit{N} was following (\ref{eq:probwinningclassicalhidden}), $  N'=S_{\mathcal{R}}\circ L'$ and $  N''=S_{\mathcal{R}}\circ L''$. Then the marginal probability for the observation to be in \textit{A} for the $ n $th round (so Alice wins) is 
\begin{align}\label{eq:jointcombinedhiddenclassical}
P_{n}^{\text{comb}}&=\int_{\mathcal{H}}  S_{A}\circ M\left(\cdots\left(S_{\mathcal{R}}\circ M\left(\left(S_{\mathcal{R}}\circ M\frac{d\nu_{0}}{d\mu}\right)\otimes\gamma\right)\right)\otimes\gamma\cdots\right) d\mu \\&=\int_{\mathcal{H}}\left(S_{A}\circ L''\circ \underbrace{N''\circ\cdots\circ N''}_{n-1}\frac{d\nu_{0}}{d\mu}\right) \;d\mu\nonumber
\end{align}
\subsection{Bounds on the extent of the paradox}
One may expect the paradox to be present to an equal or greater degree for this more general class of games. This is indeed the case, as is seen by comparing the statements of theorem \textbf{7.2.3} and \textbf{7.2.4} with the following theorem \textbf{7.3.3} and \textbf{7.3.4}. Restrict the space of pince-nez maps to those where $ N,N',N''=pN+(1-p)N' $ all have the Perron-Frobenius property, where $ N, N',N''\in\mathcal{B}\left(L^{1}(\mathcal{H};\mu)\right) $ are defined from $ L,L',L'' $ as above. Then, once again, let $ P_{A}$, $ P'_{A} $, and $ P_{A}^{\text{comb}} $ be the limits as $ n\to \infty $ of $ P_{A,n} $, $ P'_{A,n}$ and $ P_{A,n}^{\text{comb}} $ respectively. 
\paragraph*{Definition 7.3.2} The \textit{classical-hidden allowed region}, denoted $ \mathcal{CH}(A,\mathcal{R},\eta,\mathcal{H},\mu,p) $, is the set of all $\left(P_{A},P'_{A},P_{A}^{\text{comb}}\right)\in[0,1]^{\times 3} $ that occur, for fixed \textit{A}, $ \mathcal{R}$, $ \tau$, $ \mathcal{H} $, $ \mu $, and $ p $, over all allowed pince-nez maps \textit{L} and \textit{L}$ ' $. 
\medskip\\
As in the classical observed case, the existence of the paradox is then determined by the intersection of $ \mathcal{CH} $ with the cube $ \left(\frac{1}{2},1\right]\times\left(\frac{1}{2},1\right]\times\left[0,\frac{1}{2}\right) $. For $ p=1 $, $ P_{A}^{\text{comb}}=P_{A} $ and for $ p=0 $, $ P_{A}^{\text{comb}}=P'_{A} $; clearly no paradox is possible. We have the following theorems for $ p\in(0,1) $, which indicate that, once again, there are basically only two possibilities, depending on whether we have effectively a two-state hidden system or one with more than two states, as determined by the hidden base measure $ \mu $.
\paragraph*{Theorem 7.3.3} For $ p\in(0,1) $, if there are disjoint, $ \mu $-measurable subsets $ B,C,D $ with $ B\cup C\cup D=\mathcal{H} $ and $ \mu(B) $, $ \mu(C) $, and $ \mu(D) $ all strictly positive, then $ \mathcal{CH}\supset(0,1)^{\times 3} $.
\paragraph*{Proof}  Pick any $ \varepsilon>0 $ and let $ \kappa$ be the map from $ L^{1}(\mathcal{H};\mu) $ to $\mathbb{R}^{3} $ given by 
\begin{equation}
\kappa(f)=\left[\begin{array}{c}\int_{B}f\,d\mu\\\int_{C}f\,d\mu\\\int_{D}f\,d\mu\end{array} \right]
\end{equation}
Let $ h_{B} $, $ h_{C} $, and $ h_{D} $ be unit-norm functions in $ L^{1}(B;\mu)^{+} $, $ L^{1}(C;\mu)^{+} $, and $ L^{1}(D;\mu)^{+} $ respectively, each extended to all of $ \mathcal{H} $ by zero. Such functions certainly exist by the $ \sigma $-finiteness of $ \mu $. Then define the pince-nez maps \textit{L} and $L'$ by
\begin{align}
Lf&=1_{A}\otimes\left(\left[\begin{array}{ccc}h_{B}&0&0\end{array}\right]\mathbf{T}\kappa(f)\right)+1_{\tilde{A}}\otimes\left(\left[\begin{array}{ccc}0&h_{C}&h_{D}\end{array}\right]\mathbf{T}\kappa(f)\right)\\L'f&=1_{A}\otimes\left(\left[\begin{array}{ccc}h_{B}&0&0\end{array}\right]\mathbf{T}'\kappa(f)\right)+1_{\tilde{A}}\otimes\left(\left[\begin{array}{ccc}0&h_{C}&h_{D}\end{array}\right]\mathbf{T}'\kappa(f)\right)\nonumber
\end{align}
for $ \mathbf{T},\mathbf{T}' $ as in theorem \textbf{7.2.3}. Because of the properties of \textit{B}, \textit{C}, \textit{D}, $ h_{B} $, $ h_{C} $, $ h_{D} $, and $ \kappa $, the required calculation reduces to matrix products.

Then, by the deliberate construction of the maps, the row vector
\begin{equation}
\left[\begin{array}{ccc}1&1&1\end{array}\right]\mathbf{T}\left[\begin{array}{ccc}1&0&0\\0&0&0\\0&0&0\end{array}\right]= \left[\begin{array}{ccc}1&0&0\end{array}\right]
\end{equation} 
acting on the Perron-Frobenius eigenvector of \textbf{T} is its the first entry, which is indeed $ P_{A} $ for every $ s\in[0,1] $. Similarly, $ \left[\begin{array}{ccc}1&0&0\end{array}\right]\mathbf{T}' $ acting on the Perron-Frobenius eigenvector of \textbf{T}$ ' $ is its first entry, which is indeed $ P'_{A} $. For the combined game, $ P_{A}^{\text{comb}} $ is given by the row vector
\begin{equation}
\left[\begin{array}{ccc}1&1&1\end{array}\right]\left(p\mathbf{T}+(1-p)\mathbf{T}'\right)\left[\begin{array}{ccc}1&0&0\\0&0&0\\0&0&0\end{array}\right]=\left[\begin{array}{ccc}1&0&0\end{array}\right]
\end{equation}
acting on the Perron-Frobenius eigenvector of $ p\mathbf{T}+(1-p)\mathbf{T}' $, which is once again its first entry. As in theorem \textbf{7.2.3}, this varies continuously from $ 0+\mathcal{O}(\varepsilon) $ to $ 1-\mathcal{O}(\varepsilon) $ as $ \zeta $ goes from zero to one. Since $ \varepsilon $ may be taken arbitrarily small, every value for $ P_{A}^{\text{comb}}\in (0,1) $ is in the allowed region for the fixed values of $ P_{A} $ and $ P'_{A} $. $ \square $
\medskip\\
\paragraph*{Theorem 7.3.4} For $ p\in(0,1) $,if the base measure $ \mu $ is such that there is a $ \mu $-measurable subset $ B $ with $ \mu(B) $ and $ \mu(\tilde{B}) $ both strictly positive, but the conditions of the preceding theorem do not hold, then $ \mathcal{CH}(p) $ is given by the relatively open region
\[ \min\lbrace pP_{A},(1-p)P'_{A}\rbrace<P^{\text{comb}}_{A}<\max\lbrace 1-p+pP_{A},p+(1-p)P'_{A}\rbrace\]
\paragraph*{Proof} Represent measures $ \nu $ on $ \mathcal{H} $ absolutely continuous with respect to $ \mu $ by column vectors with column sum one, $ \left[\begin{array}{c}\nu(B)\\\nu(\tilde{B})\end{array}\right] $. Then all the linear maps from $ L^{1}(\mathcal{H};\mu) $ to $ L^{1}(\mathcal{H};\mu) $ are represented by $ 2\times 2 $-matrices acting by the usual matrix product.

Firstly, we will show that $ \mathcal{CH}(p) $ contains the given region. Fix any $ P_{A},P'_{A}\in(0,1] $. Then take any $ \varepsilon>0 $ sufficiently small such that the matrix  
\begin{equation}
N=\left[\begin{array}{cc}1-\left(\frac{1}{P_{A}}-1\right)\varepsilon&\varepsilon\\\left(\frac{1}{P_{A}}-1\right)\varepsilon&1-\varepsilon\end{array}\right]
\end{equation}
is stochastic. Let
\begin{equation}
L=1_{A}\otimes\left[\begin{array}{ccc}1-\left(\frac{1}{P_{A}}-1\right)\varepsilon&&0\\\left(\frac{1}{P_{A}}-1\right)\varepsilon&&0\end{array}\right]+1_{\tilde{A}}\otimes\left[\begin{array}{cc}0&\varepsilon\\0&1-\varepsilon\end{array}\right]
\end{equation}
and, for $ s\in[0,1] $, 
\begin{equation}
N'=\left[\begin{array}{cc}\frac{1}{2}(1+s)&\frac{1}{2}s\\\frac{1}{2}(1-s)&1-\frac{1}{2}s\end{array}\right],L'=P'_{A}1_{A}\otimes\, N'+(1-P'_{A})1_{\tilde{A}}\otimes N'
\end{equation}

Then $ \left[\begin{array}{cc}1&1\end{array}\right] S_{A} \circ L= \left[\begin{array}{cc}1&0\end{array}\right] $ acting on the Perron-Frobenius eigenvector of \textit{N} is its first entry, which is indeed $ P_{A} $ by the deliberate construction of the maps. Similarly, $ \left[\begin{array}{cc}1&1\end{array}\right] S_{A}\circ L'=P'_{A}\left[\begin{array}{cc}1&1\end{array}\right] $ acting on the Perron-Frobenius eigenvector of $ N' $ is indeed $ P'_{A} $ for all \textit{s}. For the combined game, $ P_{A}^{\text{comb}} $ is given by
\begin{equation}
\left[\begin{array}{cc}1&1\end{array}\right]S_{A}\circ\left(pL+(1-p)L'\right)=p\left[\begin{array}{cc}1&0\end{array}\right]+(1-p)P'_{A}\left[\begin{array}{cc}1&1\end{array}\right]
\end{equation}
acting on the Perron-Frobenius eigenvector of $ pN+(1-p)N' $. This varies continuously from $ (1-p)P'_{A}+\mathcal{O}(\varepsilon) $ to $ p+(1-p)P'_{A}-\mathcal{O}(\varepsilon) $ as $ s $ goes from zero to one. Since $ \varepsilon $ may be taken arbitrarily small, every value in the interval $ \left((1-p)P'_{A},p+(1-p)P'_{A}\right) $ can be taken by $ P_{A}^{\text{comb}} $ for the fixed values of $ P_{A} $ and $ P'_{A} $. Repeating the process with primed$ \leftrightarrow $unprimed and $ p\leftrightarrow 1-p $, every value in the interval $ \left(pP_{A},1-p+pP_{A}\right) $ can be taken by $ P_{A}^{\text{comb}} $ for the fixed values of $ P_{A} $ and $ P'_{A} $. A similar argument using appropriately modified maps holds for either $ P_{A} $ or $ P'_{A} $ or both of them being zero. 

Now, we will show that $ \mathcal{CH}(p) $ is contained in the given region. A key observation is that instead of varying over all maps $ S_{A}\circ L $ and $ S_{A}\circ L $ with positive entries subject to the constraint that $ N=S_{\mathcal{R}}\circ L $ is stochastic, one may equivalently vary over all stochastic maps \textit{N} and row vectors $ \mathbf{v} $ with entries in $ [0,1] $ (with $ \mathbf{v}=\left[\begin{array}{cc}1&1\end{array}\right] S\circ L $). The same situation holds for the primed maps. Write $ \mathbf{v}=\left[\begin{array}{cc}a&b\end{array}\right] $, $ N=\left[\begin{array}{cc}1-c&d\\c&1-d\end{array}\right] $, $ \mathbf{v}'=\left[\begin{array}{cc}a'&b'\end{array}\right] $, and $ N'=\left[\begin{array}{cc}1-c'&d'\\c'&1-d'\end{array}\right] $, with $ a,b,c,d,a',b',c',d'\in[0,1] $ except $ c=d=0 $, $ c=d=1 $, $ c'=d'=0 $, and $ c'=d'=1 $ are not allowed since the maps must have the Perron-Frobenius property. Fixing the values of $ P_{A} $ and $ P'_{A} $ and using explicit expressions for the Perron-Frobenius eigenvector gives the optimization problem:
\begin{align}
&\text{constraints: }ad+bc= P_{A}(c+d),a'd'+b'c'= P'_{A}(c'+d')\\&\text{extremize: }P^{\text{comb}}_{A}=\dfrac{\left(pa+(1-p)a'\right)\left(pd+(1-p)d'\right)+\left(pb+(1-p)b'\right)\left(pc+(1-p)c'\right)}{p(c+d)+(1-p)(c'+d')}\nonumber
\end{align} 
The quantity to be extremized is a rational linear function of $ c,d,c',d' $; furthermore, the constraints are homogeneous in the sense that they are unaffected by $ c\to\xi c $, $ d\to\xi d $ for any positive $ \xi $ and $ c'\to\xi' c' $, $ d'\to\xi' d' $ for any positive $ \xi' $. Therefore, the extreme values can only be attained as either $ c,d\to 0 $ or $ c',d'\to 0 $. In the first case, using the remaining condition, the quantity to be extremized is $(1-p)P'_{A}+\dfrac{p(ad'+bc')}{(c'+d')} $. The term on the right is between 0 and \textit{p}. In the second case, using the remaining condition, the quantity to be extremized is $pP_{A}+\dfrac{(1-p)(a'd+b'c)}{(c+d)} $. The term on the right is between 0 and $ 1-p $. The actual extreme values cannot be attained because the maps corresponding to those parameter values are not allowed. $ \square $
\section{Defining a quantum analogue of the Markov model}\label{sec:quantum}
\subsection{An analogous game}
As we showed in \S\ref{sec:quantumnodes}, one may consider the analogous game to the above one employing maps on density-matrices rather than maps on measures. This leads to the following Bayesian network model:
\paragraph*{Definition 7.4.1} A \textit{Markov-Bayesian-quantum model} ($ \mathcal{R} $, $ \eta $, \textsf{H}, \textit{L}, $ \rho_{0} $) is composed of: an observation set $ \mathcal{R} $ with base measure $ \eta $, a Hilbert space \textsf{H}, a pince-nez map\\$ L\in\mathcal{B}\left(\mathcal{D}(\mathsf{H}), L^{1}(\mathcal{R};\eta;\mathcal{D}(\mathsf{H}))\right) $ that is norm-preserving (on the positive cone) and completely-positive, and an initial density-matrix $\rho_{0}$ on \textsf{H} with $ \text{tr }\rho_{0}=1 $.
\medskip\\
The use of the word \textit{quantum} will be justified below. The accompanying graphical model is (note it is the same as (\ref{fig:hiddengame}), illustrating the analogy graphically):
\begin{align}\label{fig:quantumBayes}
\setlength{\unitlength}{.8 in}
\begin{picture}(5.5,.8)
\color{blue}
\put(.1,.1){\oval(.2,.2)[r]}
\put(0,.2){\line(1,0){.1}}
\put(0,0){\line(1,0){.1}}
\put(0,0){\line(0,1){.2}}
\put(1,.1){\circle{.2}}
\put(2,.1){\circle{.2}}
\put(3.5,.1){\circle{.2}}
\put(4.5,.1){\circle{.2}}
\put(5.5,.1){\oval(.2,.2)[l]}
\put(5.5,.2){\line(1,0){.1}}
\put(5.5,0){\line(1,0){.1}}
\put(5.6,0){\line(0,1){.2}}
\put(.2,.1){\vector(1,0){.7}}
\put(1.09,.1){\vector(1,0){.8}}
\put(2.09,.1){\line(1,0){.5}}
\put(2.7,.05){$\cdots$}
\put(2.89,.1){\vector(1,0){.5}}
\put(3.59,.1){\vector(1,0){.8}}
\put(4.59,.1){\vector(1,0){.8}}
\put(.89,.1){\line(0,1){.1}}
\put(1.89,.1){\line(0,1){.1}}
\put(3.39,.1){\line(0,1){.1}}
\put(4.39,.1){\line(0,1){.1}}
\color{black}
\put(1,.3){\circle{.2}}
\put(2,.3){\circle{.2}}
\put(3.5,.3){\circle{.2}}
\put(4.5,.3){\circle{.2}}
\put(1,.45){1}
\put(2,.45){2}
\put(3.5,.45){$ n-1 $}
\put(4.5,.45){\textit{n}}
\put(4.4,.3){\line(1,0){.19}}
\put(4.5,.209){\line(0,1){.185}}
\put(.89,.2){\line(0,1){.1}}
\put(1.89,.2){\line(0,1){.1}}
\put(3.39,.2){\line(0,1){.1}}
\put(4.39,.2){\line(0,1){.1}}
\end{picture}
\end{align}
Then the joint probability to observe $ (x_{1},x_{2},\ldots,x_{n})\in A_{1}\times A_{2}\times\cdots\times A_{n} $, for any $ \eta $-measurable $ A_{1}, A_{2},\ldots, A_{n}\in\mathcal{R} $, is (compare to (\ref{eq:jointclasicalhiddenchain}))
\begin{equation}
\text{tr }S_{A_{n}}\circ L\circ\cdots \circ S_{A_{1}}\circ L\rho_{0} 
\end{equation}
for $ S_{A}\in \mathcal{B}\left( L^{1}(\mathcal{R};\eta;\mathcal{D}(\mathsf{H})),\mathcal{D}(\mathsf{H})\right) $ the linear map given by the integration $ S_{A}\varphi=\int_{A}\varphi\,d\eta $.

Employing this model for the game, then the marginal probability for the observation to be in \textit{A} at the $ n $th round (so Alice wins) is (compare to (\ref{eq:probwinningclassicalhidden})) 
\begin{equation}\label{eq:probwinningquantum}
P_{A,n}=\text{tr }S_{A}\circ L \circ\underbrace{N\circ\cdots\circ N}_{n-1}\rho_{0}
\end{equation}
where $ N\in\mathcal{B}\left(\mathcal{D}(\mathsf{H})\right)  $ is defined as the map $  S_{\mathcal{R}}\circ L $. Because of the definition of the game, it is possible to reduce to the case where the event space for $ \mathcal{R} $ is simply $ \mathcal{E}=\lbrace\varnothing, A,\tilde{A},\mathcal{X}\rbrace $ and its base measure $ \eta $ is the measure with $ \eta(A)=\eta(\tilde{A})=1 $.
\subsection{An alternate game using textbook quantum mechanics}
Consider the following quantum game that is a generalization of that employed by~\cite{flitney}, but using our simpler winning criterion.
\paragraph*{Definition 7.4.2} A \textit{Markov-quantum process} (\textsf{H}, \textit{q}, \textit{U}) with: Hilbert space \textsf{H}, number of \textit{quantum channels} \textit{q}, and unitary operator $ U:\mathsf{H}^{\otimes q}\to \mathsf{H}^{\otimes q} $--is the operator 
\[\psi\to \left(I_{\mathsf{H}^{\otimes(q-1)(n-1)}}\otimes U \right)\cdots\left(I_{\mathsf{H}^{\otimes (q-1)}}\otimes U\otimes I_{\mathsf{H}^{\otimes(q-1)(n-2)}} \right)\left(U\otimes I_{\mathsf{H}^{\otimes(q-1)(n-1)}} \right) \psi\]
for any $\psi\in\mathsf{H}^{\otimes((q-1)n+1)}$.
\medskip\\
The corresponding quantum circuit for the case of $ q=4 $ is: 
\begin{align}\label{fig:quantumcircuit}
\setlength{\unitlength}{.75 in}
\begin{picture}(5.5,2.2)
\put(0,1){\oval(.1,2)}
\put(5,1){\oval(.1,2)}
\put(1,1.7){\oval(.1,.6)}
\put(2,1.2){\oval(.1,.6)}
\put(4,.3){\oval(.1,.6)}
\put(.05,1.9){\line(1,0){.9}}
\put(.05,1.75){\line(1,0){.9}}
\put(.05,1.6){\line(1,0){.9}}
\put(.05,1.45){\line(1,0){.9}}
\put(.05,1.3){\line(1,0){1.9}}
\put(.05,1.15){\line(1,0){1.9}}
\put(.05,1){\line(1,0){1.9}}
\put(3.5,.55){\line(1,0){.45}}
\put(.05,.4){\line(1,0){3.9}}
\put(.05,.25){\line(1,0){3.9}}
\put(.05,.1){\line(1,0){3.9}}
\put(4.05,.55){\line(1,0){.9}}
\put(4.05,.4){\line(1,0){.9}}
\put(4.05,.25){\line(1,0){.9}}
\put(4.05,.1){\line(1,0){.9}}
\put(1.05,1.9){\line(1,0){3.9}}
\put(1.05,1.75){\line(1,0){3.9}}
\put(1.05,1.6){\line(1,0){3.9}}
\put(1.05,1.45){\line(1,0){.9}}
\put(2.05,1.45){\line(1,0){2.9}}
\put(2.05,1.3){\line(1,0){2.9}}
\put(2.05,1.15){\line(1,0){2.9}}
\put(2.05,1){\line(1,0){.5}}
\put(1,.7){$ \vdots $}
\put(1,.45){$ \vdots $}
\put(2.4,.6){$ \ddots $}
\put(3.2,.5){$ \cdots $}
\put(2.6,.95){$ \cdots $}
\put(4.5,.85){$ \vdots $}
\put(4.5,.6){$ \vdots $}
\put(5.1,1.9){q1}
\put(5.1,1.73){q2}
\put(5.1,1.56){q3}
\put(5.1,1.39){q4}
\put(5.1,1.22){q5}
\put(5.1,1.05){q6}
\put(5.1,.56){q$ (3n-2) $}
\put(5.1,.39){q$ (3n-1) $}
\put(5.1,.22){q$ (3n) $}
\put(5.1,.05){q$ (3n+1) $}
\end{picture}
\end{align}
This may be compared to the quantum process with accompanying quantum circuit employed in~\cite{flitney}.

Let $ \lbrace P_{A_{1}\times\cdots\times A_{n}}\rbrace $ over all $ \tau $-measurable $ A_{1},\ldots,A_{n} $ be a complete set of mutually commuting, orthogonal projectors\footnote{A complete set of mutually commuting, orthogonal projectors relative to a base measure $ \mu $ is defined similarly with that relative to a $ \sigma $-algebra except the condition $ E_{\varnothing}=0 $ is replaced by the condition that $ \mu(B)=0\Rightarrow E_{B}=0 $.} on $ \mathsf{H}^{\otimes((q-1)n+1)} $.

A textbook quantum model is then provided by the following:
\paragraph*{Definition 7.4.3} A \textit{Markov-quantum-model} ($ \mathcal{R} $, $ \tau $, \textsf{H}, \textit{q}, \textit{U}, $ \lbrace P_{A_{1}\times\cdots\times A_{n}}\rbrace $, $ \psi_{i} $) is composed of: an observation set $ \mathcal{R} $ with base measure $ \tau $, a Markov-quantum process (\textsf{H}, \textit{q}, \textit{U}), a collection of orthogonal projectors $\lbrace P_{A_{1}\times\cdots\times A_{n}}\rbrace$ as described above, and an initial length-one vector $ \psi_{i}\in \mathsf{H}^{\otimes ((q-1)n+1)} $.
\medskip\\
The joint probability to observe $(x_{1},x_{2},\ldots,x_{n})\in A_{1}\times A_{2}\times\cdots\times A_{n}$ is then $ \left\Vert P_{A_{1}\times\cdots\times A_{n}}\psi_{f}\right\Vert^{2} $, where $ \psi_{f} $ is given by applying the Markov-quantum process to $ \psi_{i} $. In particular, the marginal probability for the observation to be in \textit{A} at the $ n $th round (so Alice wins) is $ P_{A,n}=\left\Vert P_{\mathcal{X}\times\cdots\times\mathcal{X}\times A}\psi_{f}\right\Vert^{2} $.
\subsection{Equivalence of the two models}
Start with any Markov-quantum model. The joint probability to observe $ (x_{1},x_{2},\ldots,x_{n})$  in $ A_{1}\times\cdots\times A_{n}$ is given by
\begin{equation}\label{eq:tracemarkovmodel}
\left\Vert P_{A_{1}\times\cdots\times A_{n}}\psi_{f}\right\Vert^{2}=\langle P_{A_{1}\times\cdots\times A_{n}}\psi_{f},\psi_{f}\rangle=\text{tr }P_{A_{1}\times\cdots\times A_{n}}\psi_{f}\psi_{f}^{*}
\end{equation}
This has a graphical representation as the following tensor network (illustrated for $ q=4 $):
\begin{align}\label{fig:tensornetwork}
\setlength{\unitlength}{.75 in}
\begin{picture}(5.5,2.2)
\put(0,1.9){\circle{.1}}
\put(0,1.6){\oval(.1,.4)}
\put(0,1.15){\oval(.1,.4)}
\put(0,.25){\oval(.1,.4)}
\put(5,1.9){\circle{.1}}
\put(5,1.6){\oval(.1,.4)}
\put(5,1.15){\oval(.1,.4)}
\put(5,.25){\oval(.1,.4)}
\put(.5,1.7){\oval(.1,.6)}
\put(1,1.2){\oval(.1,.6)}
\put(2,.3){\oval(.1,.6)}
\put(4.5,1.7){\oval(.1,.6)}
\put(4,1.2){\oval(.1,.6)}
\put(3,.3){\oval(.1,.6)}
\put(2.5,1.75){\oval(.1,.4)}
\put(2.5,1.3){\oval(.1,.4)}
\put(2.5,.4){\oval(.1,.4)}
\put(.05,1.9){\line(1,0){.4}}
\put(.05,1.75){\line(1,0){.4}}
\put(.05,1.6){\line(1,0){.4}}
\put(.05,1.45){\line(1,0){.4}}
\put(4.95,1.9){\line(-1,0){.4}}
\put(4.95,1.75){\line(-1,0){.4}}
\put(4.95,1.6){\line(-1,0){.4}}
\put(4.95,1.45){\line(-1,0){.4}}
\put(.55,1.9){\line(1,0){1.9}}
\put(.55,1.75){\line(1,0){1.9}}
\put(.55,1.6){\line(1,0){1.9}}
\put(4.45,1.9){\line(-1,0){1.9}}
\put(4.45,1.75){\line(-1,0){1.9}}
\put(4.45,1.6){\line(-1,0){1.9}}
\put(.55,1.45){\line(1,0){.4}}
\put(4.45,1.45){\line(-1,0){.4}}
\put(.05,1.3){\line(1,0){.9}}
\put(.05,1.15){\line(1,0){.9}}
\put(.05,1){\line(1,0){.9}}
\put(4.95,1.3){\line(-1,0){.9}}
\put(4.95,1.15){\line(-1,0){.9}}
\put(4.95,1){\line(-1,0){.9}}
\put(1.05,1.45){\line(1,0){1.4}}
\put(1.05,1.3){\line(1,0){1.4}}
\put(1.05,1.15){\line(1,0){1.4}}
\put(3.95,1.45){\line(-1,0){1.4}}
\put(3.95,1.3){\line(-1,0){1.4}}
\put(3.95,1.15){\line(-1,0){1.4}}
\put(1.05,1){\line(1,0){.4}}
\put(3.95,1){\line(-1,0){.4}}
\put(1.5,1){$\ldots$}
\put(3.25,1){$\ldots$}
\put(.05,.4){\line(1,0){1.9}}
\put(.05,.25){\line(1,0){1.9}}
\put(.05,.1){\line(1,0){1.9}}
\put(4.95,.4){\line(-1,0){1.9}}
\put(4.95,.25){\line(-1,0){1.9}}
\put(4.95,.1){\line(-1,0){1.9}}
\put(2.05,.1){\line(1,0){.9}}
\put(2.05,.55){\line(1,0){.4}}
\put(2.05,.4){\line(1,0){.4}}
\put(2.05,.25){\line(1,0){.4}}
\put(2.95,.55){\line(-1,0){.4}}
\put(2.95,.4){\line(-1,0){.4}}
\put(2.95,.25){\line(-1,0){.4}}
\put(1.95,.55){\line(-1,0){.4}}
\put(3.05,.55){\line(1,0){.4}}
\put(1.25,.55){$\ldots$}
\put(3.55,.55){$\ldots$}
\put(0,.6){$ \vdots $}
\put(5,.6){$ \vdots $}
\put(2.5,.75){$ \vdots $}
\put(1.5,.7){$ \ddots $}
\put(3.5,.7){$ \iddots $}
\put(5.1,1.9){q1}
\put(5.1,1.73){q2}
\put(5.1,1.56){q3}
\put(5.1,1.39){q4}
\put(5.1,1.22){q5}
\put(5.1,1.05){q6}
\put(5.1,.88){q7}
\put(5.1,.39){q$ (3n-1) $}
\put(5.1,.22){q$ (3n) $}
\put(5.1,.05){q$ (3n+1) $}
\end{picture}
\end{align}
The initial wavefunction $ \psi_{i}=\psi_{0}\otimes(\psi_{1})^{\otimes n} $ is on the left, with its conjugate on the right. The unitary operators $ U $ are on the left diagonal, with the adjoints $ U^{*} $ on the right diagonal. The projectors are down the center.

Rather than performing the calculation in the difficult manner (left-to-right), the calculation can be done the easy way (top-to-bottom). This reordering gives rise to the following graphical model for a Bayesian network, where the labels indicate where the quantum channels from the quantum circuit and tensor network models go in the latter:
\begin{align}
\setlength{\unitlength}{.7 in}
\begin{picture}(5.9,2.2)
\color{blue}
\put(.5,1){\oval(.2,.2)[r]}
\put(.4,1.1){\line(1,0){.1}}
\put(.4,.9){\line(1,0){.1}}
\put(.4,.9){\line(0,1){.2}}
\put(1,1){\circle{.2}}
\put(1,.2){\oval(.2,.2)[t]}
\put(.9,.2){\line(0,-1){.1}}
\put(1.1,.2){\line(0,-1){.1}}
\put(.9,.1){\line(1,0){.2}}
\put(1.5,1){\oval(.1,.3)}
\put(2,1){\circle{.2}}
\put(2,.2){\oval(.2,.2)[t]}
\put(1.9,.2){\line(0,-1){.1}}
\put(2.1,.2){\line(0,-1){.1}}
\put(1.9,.1){\line(1,0){.2}}
\put(2.5,1){\oval(.1,.3)}
\put(4,1){\circle{.2}}
\put(4,.2){\oval(.2,.2)[t]}
\put(3.9,.2){\line(0,-1){.1}}
\put(4.1,.2){\line(0,-1){.1}}
\put(3.9,.1){\line(1,0){.2}}
\put(4.5,1){\oval(.1,.3)}
\put(2.01,1.7){\oval(.2,.2)[l]}
\put(2.01,1.8){\line(1,0){.1}}
\put(2.01,1.6){\line(1,0){.1}}
\put(2.11,1.6){\line(0,1){.2}}
\put(3.01,1.7){\oval(.2,.2)[l]}
\put(3.01,1.8){\line(1,0){.1}}
\put(3.01,1.6){\line(1,0){.1}}
\put(3.11,1.6){\line(0,1){.2}}
\put(5.02,1.7){\oval(.2,.2)[l]}
\put(5.02,1.8){\line(1,0){.1}}
\put(5.02,1.6){\line(1,0){.1}}
\put(5.12,1.6){\line(0,1){.2}}
\put(5,1){\oval(.2,.2)[l]}
\put(5,1.1){\line(1,0){.1}}
\put(5,.9){\line(1,0){.1}}
\put(5.1,.9){\line(0,1){.2}}
\put(.59,1){\vector(1,0){.32}}
\put(1.09,1){\vector(1,0){.35}}
\put(1.55,1){\vector(1,0){.35}}
\put(1.55,1.1){\vector(1,2){.35}}
\put(2.09,1){\vector(1,0){.35}}
\put(2.55,1){\vector(1,0){.35}}
\put(2.55,1.1){\vector(1,2){.35}}
\put(4.09,1){\vector(1,0){.35}}
\put(4.55,1){\vector(1,0){.35}}
\put(4.55,1.1){\vector(1,2){.35}}
\put(1,.3){\vector(0,1){.6}}
\put(2,.3){\vector(0,1){.6}}
\put(4,.3){\vector(0,1){.6}}
\put(3,1){$\cdots$}
\put(3.3,1){$\cdots$}
\put(.6,1.05){0}
\put(1.15,1.05){1}
\put(2.15,1.05){2}
\put(4.15,1.05){\textit{n}}
\put(3.5,1){\vector(1,0){.4}}
\put(1.9,1.7){\line(0,1){.1}}
\put(2.9,1.7){\line(0,1){.1}}
\put(4.9,1.7){\line(0,1){.1}}
\color{black}{\put(2,1.9){\circle{.2}}}
\put(3,1.9){\circle{.2}}
\put(5,1.9){\circle{.2}}
\put(2,2.05){1}
\put(3,2.05){2}
\put(5,2.05){\textit{n}}
\put(.5,.8){q1}
\put(1.12,.25){q2,q3,}
\put(1.12,.05){q4}
\put(2.12,.25){q5,q6,}
\put(2.12,.05){q7}
\put(4.12,.25){q$ (3n-1)$,q$ (3n) $,}
\put(4.12,.05){q$ (3n+1) $}
\put(2.15,1.8){q1,q2,}
\put(2.15,1.6){q3}
\put(3.15,1.8){q4,q5,}
\put(3.15,1.6){q6}
\put(5.15,1.8){q$ (3n-2) $,}
\put(5.15,1.6){q$ (3n-1) $,}
\put(5.15,1.4){q$ (3n) $}
\put(5.15,.95){q$ (3n+1) $}
\put(5,2.05){\textit{n}}
\put(1.9,1.9){\line(1,0){.19}}
\put(2,1.809){\line(0,1){.185}}
\put(2.9,1.9){\line(1,0){.19}}
\put(3,1.809){\line(0,1){.185}}
\put(4.9,1.9){\line(1,0){.19}}
\put(5,1.809){\line(0,1){.185}}
\put(1.9,1.8){\line(0,1){.1}}
\put(2.9,1.8){\line(0,1){.1}}
\put(4.9,1.8){\line(0,1){.1}}
\end{picture}
\end{align}
By replacing each repeated module by a pince-nez, this becomes (\ref{fig:quantumBayes}). (Note the efficiency of the graphical model for the Bayesian network compared to the tensor network--there is no need to place every operator and initial condition twice in the graph.) The preceding graphical manipulation inspires the following:
\paragraph*{Theorem 7.4.4} If a Markov-quantum model is of the form
\[\left( \mathcal{R} ,\tau,\mathsf{H}, q, U, \lbrace Q_{A_{1}}\otimes \cdots\otimes Q_{A_{n}}\otimes I_{\mathsf{H}}\rbrace , \psi_{0}\otimes(\psi_{1}^{\otimes n}) \right) \]
for some unit-length vectors $ \psi_{0}\in\mathsf{H} $ and $ \psi_{1}\in\mathsf{H}^{\otimes (q-1)} $ and collection of orthogonal projectors $ \lbrace Q_{C}\rbrace_{C\in \mathcal{E}} $ on $ \mathsf{H}^{\otimes (q-1)} $, then there is an equivalent (in the sense of giving the same joint probabilities) Markov-Bayesian-quantum model ($ \mathcal{R} $, $ \tau $, \textsf{H}, \textit{L}, $ \rho_{0} $).
\paragraph*{Proof} Start with any such Markov-quantum model. The joint probability to observe $ (x_{1},x_{2},\ldots,x_{n})$  in $ A_{1}\times\cdots\times A_{n}$ is given by \begin{equation}
\left\Vert P_{A_{1}\times\cdots\times A_{n}}\psi_{f}\right\Vert^{2}=\langle P_{A_{1}\times\cdots\times A_{n}}\psi_{f},\psi_{f}\rangle=\text{tr }P_{A_{1}\times\cdots\times A_{n}}\psi_{f}\psi_{f}^{*}
\end{equation}
Write the trace as the tensor product of reduced traces,
\begin{equation}
\text{tr}_{\mathsf{H}^{\otimes((q-1)n+1)}}=\left(\text{tr}_{\mathsf{H}^{\otimes (q-1)}}\right)^{\otimes n}\otimes \text{tr}_{\mathsf{H}}
\end{equation}
This tensor product of maps is well-defined using \textbf{A1.3}, \textbf{B4.1}, \textbf{B5.5}, and \textbf{B5.8}. Using the given forms, $ P_{A_{1}\times\cdots\times A_{n}}=Q_{A_{1}}\otimes \cdots\otimes Q_{A_{n}}\otimes I_{\mathsf{H}} $ and $ \psi_{i}=\psi_{0}\otimes(\psi_{1}^{\otimes n}) $, then ``pushing" the partial traces into the expression as far as possible gives the joint probability as
\begin{equation}
\begin{array}{c}
\left(K(\cdot;A_{n})\otimes \text{tr}_{\mathsf{H}}\right)\left(U\left(\left(\left(K(\cdot;A_{n-1})\otimes I_{\mathcal{B}(\mathsf{H})}\right)\left(\cdots\right.\right.\right.\right.\\\\\left(K(\cdot;A_{2})\!\otimes\!\! I_{\mathcal{B}(\mathsf{H})}\right)\!\left(\!U\!\left(\left(\left(K(\cdot;A_{1})\!\otimes\!\! I_{\mathcal{B}(\mathsf{H})}\right)(U(\psi_{0}\psi_{0}^{*}\!\otimes\! \left(\psi_{1}\psi_{1}^{*}\right))U^{*})\right)\!\otimes\!\left(\psi_{1}\psi_{1}^{*}\right)\right)\!U^{*}\!\right)\\\\\left.\left.\left.\left.\cdots\right)\right)\otimes\left(\psi_{1}\psi_{1}^{*}\right)\right)U^{*}\right)\end{array}
\end{equation}
where $I_{\mathcal{B}(\mathsf{H})}  $ is the identity map on operators in $ \mathcal{B}(\mathsf{H}) $ and
\begin{equation}
K:\mathcal{D}\left(\mathsf{H}^{\otimes (q-1)}\right)\times\left(\begin{array}{l}\tau-\text{measurable}\\\text{subsets of }\mathcal{R}\end{array}\right)\to\mathbb{R}
\end{equation}
is given by $ K(\rho;C)=\text{tr }Q_{C} \rho $. The various tensor products of maps in the expression are still well-defined by the above propositions. \textit{K} is countably-additive in its second argument by the countable-additivity of the projectors $ \lbrace Q_{C}\rbrace $ (with convergence in the weak* topology). $ K(\cdot;C) $ is manifestly completely-positive for any $ C\in\mathcal{E} $. Then, by \textbf{B5.5}, and \textbf{B5.8}, $ \Vert K(\cdot;C)\otimes I_{\mathcal{B}(\mathsf{H})}\Vert_{\text{op}}=\Vert K(\cdot;C)\Vert_{\text{op}} $. Therefore, for any fixed $ \rho\in \mathcal{D}\left(\mathsf{H}^{\otimes (q-1)}\right)^{+} $, $ K(\rho;\cdot) $ is a measure on $ \mathcal{R} $. Furthermore, this measure is clearly absolutely continuous with respect to $ \tau $ since $ Q_{C}=0 $ if $ \tau(C)=0 $.

Let $N: \mathcal{D}\left(\mathsf{H}\right)\times\mathcal{E}\to \mathcal{D}\left(\mathsf{H}\right) $ be the map given by
\begin{equation}
MN\rho;C)=\left(K(\cdot;C)\otimes I_{\mathcal{B}(\mathsf{H})}\right)(U(\rho\otimes\left(\psi_{1}\psi_{1}^{*}\right))U^{*})
\end{equation}
By the above properties of \textit{K}, for any fixed $ \rho\in \mathcal{D}\left(\mathsf{H}\right)^{+} $, $ N(\rho;\cdot) $ is a $ \mathcal{D}\left(\mathsf{H}\right)^{+} $-valued vector measure on $ \mathcal{R} $ that is absolutely continuous with respect to $ \tau $. $ \mathcal{D}\left(\mathsf{H}\right) $ has the Radon-Nikod\'{y}m property, so $  N(\rho;\cdot) $ has Radon-Nikod\'{y}m derivative $ \frac{dN(\rho;\cdot)}{d\tau}\in L^{1}(\mathcal{R};\tau;\mathcal{D}\left(\mathsf{H}\right)^{+}) $ with the property that $N(\rho;C)=\int_{C} \frac{dN(\rho;\cdot)}{d\tau}\;d\tau  $ for any $ \tau $-measurable subset \textit{C}. Then define the pince-nez map \textit{L} by $ L\rho= \frac{dN(\rho;\cdot)}{d\tau}$. The required completely-positive and norm-preserving (on the positive cone) properties of \textit{L} are readily demonstrated. $ \square $
\medskip\\

More remarkable (and requiring  theorem \textbf{5.1.1} to prove) is the following result:
\paragraph*{Theorem 7.4.5} If a Markov-Bayesian-quantum model is of the form ($ \mathcal{R} $, $ \tau $, \textsf{H}, \textit{L}, $ \psi_{0}\psi_{0}^{*} $), then there is an equivalent (in the sense of giving the same joint probabilities) Markov-quantum-model 
\[\left( \mathcal{R}' ,\tau',\mathsf{H}, q, U, \lbrace P_{A_{1}\times \cdots\times A_{n}}\rbrace , \psi_{i} \right) \]
\paragraph*{Proof} Start with any such Markov-Bayesian-quantum model. From theorem \textbf{5.1.1} and the Radon-Nikod\'{y}m property of $ \mathcal{D}(\mathsf{H}) $, \textit{L} can be written in terms of the Radon-Nikod\'{y}m derivative, $ L\rho=\frac{dN(\rho;\cdot)}{d\tau} $, with 
\begin{equation}
N(\rho;B)=\left(\text{tr}_{\mathsf{M}}\otimes \Phi(B)\otimes I_{\mathcal{B}(\mathsf{H})}\right) \left(V\rho V^{*}\right)
\end{equation}
for some Hilbert space \textsf{M}, some partial isometry $ V:L^{2}(\mathsf{H})\to \mathsf{M}\otimes L^{2}(\mathcal{R};\tau)\otimes \mathsf{H}  $, and where $ \Phi(B) $ is the functional on $ \mathcal{D}(L^{2}(\mathcal{R};\tau)) $ given by $ \Phi(B)\tau=\int_{ B}\text{diag }\tau\;d\nu $. Furthermore, by the theorem, if the Hilbert space \textsf{H} has finite dimension, the dimension of \textsf{M} equal to $ (\dim\mathsf{H})^{2}$.

The dimension of $ L^{2}(\mathcal{R};\tau) $ then determines the minimum number of quantum channels, \textit{q}. If $\dim L^{2}(\mathcal{R};\tau)\leq (\dim\mathsf{H}) $, take $ q=4 $. If $ \dim\mathsf{H}<\dim L^{2}(\mathcal{R};\tau)\leq (\dim\mathsf{H})^{2} $, take $ q=5 $. If $ (\dim\mathsf{H})^{2}<\dim L^{2}(\mathcal{R};\tau)\leq (\dim\mathsf{H})^{3} $, take $ q=6 $. For any of these three cases, take $ Q $ to be any partial isometry from $  L^{2}(\mathcal{R};\tau) $ to $ \mathsf{H}^{\otimes(q-3)} $. For $ (\dim\mathsf{H})^{3}<\dim L^{2}(\mathcal{R};\tau) $, let \textsf{G} be the subspace of $ L^{2}(\mathcal{R};\tau) $ which is relevant, given by the norm-closure of the span of $ \left\lbrace \left(\psi^{*}\otimes\pi(1)\otimes\xi^{*}\right)V\phi\left\vert\phi,\psi\in\mathsf{H},\xi\in\mathsf{M}\right.\right\rbrace $. Then $ \dim\mathsf{G}\leq (\dim\mathsf{H})^{2}\dim\mathsf{M}= (\dim\mathsf{H})^{4} $, so take $ q=7 $ and $ Q $ to be any partial isometry from $ \mathsf{G} $ to $ \mathsf{H}^{\otimes 4}$.

Now select any unit-length $ \psi_{1}\in\mathsf{H}^{\otimes (q-1)} $ and any partial isometry $ R:\mathsf{K}\to\mathsf{H}\otimes \mathsf{H} $. Then there is some unitary $ U:\mathsf{H}^{\otimes q}\to \mathsf{H}^{\otimes q} $ such that
\begin{equation}
 U(\phi\otimes \psi_{1})=(R\otimes Q\otimes I_{\mathsf{H}})V\phi \text{ for every }\phi\in\mathsf{H}
\end{equation}
Hence, by the spectral theorem for compact operators,
\begin{equation}
 U(\rho\otimes \psi_{1}\psi_{1}^{*})U^{*}=(R\otimes Q\otimes I_{\mathsf{H}})V\rho V^{*}(R^{*}\otimes Q^{*}\otimes I_{\mathsf{H}} )\text{ for every }\rho\in\mathcal{D}(\mathsf{H})^{+}
\end{equation}
Take $ \psi_{i}=\psi_{0}\otimes (\psi_{1}^{\otimes n}) $. Finally, if $ \dim L^{2}(\mathcal{X};\mu)=(\dim\mathsf{H})^{q-3} $ or $ \dim\mathsf{G}=(\dim\mathsf{H})^{4} $, take $ \mathcal{X}'=\mathcal{X} $, $ \tau'=\tau $, and $ P_{A_{1}\times\cdots\times A_{n}} $ to be
\begin{equation}
\left( I_{\mathsf{H}^{\otimes 2}}\!\otimes\!Q \pi(1_{A_{1}})Q^{*}\right)\otimes\cdots\otimes\left( I_{\mathsf{H}^{\otimes 2}}\!\otimes\!Q \pi(1_{A_{n}})Q^{*}\right)\!\otimes\! I_{\mathsf{H}}\hspace{.1 in }
\end{equation}
Otherwise, add one point $ x_{0} $ to $ \mathcal{X} $ to form $ \mathcal{X}' $. Add an atom of weight one at $ x_{0} $ to $ \tau $ to form $ \tau' $. For $ A_{1},\ldots, A_{n}\in\mathcal{E} $, let $ P_{A_{1}\times\cdots\times A_{n}} $ be defined as above. Replacing any of the $ A_{j} $'s with $ \lbrace x_{0}\rbrace $, replace $ Q \pi(1_{A_{j}})Q^{*} $ with $ I_{\mathsf{H}^{\otimes(q-3})}-Q^{*}Q $. (Note that with the given initial wavefunction and time-evolution, the probabilities for observing $ \lbrace x_{0}\rbrace $ are all zero--it is only added so the projectors form a complete set with $ P_{{\mathcal{X}'}^{\times n}}=I_{\mathsf{H}^{\otimes((q-1)n+1}} $.) $ \square $
\section{Parrondo's paradox for the quantum game}\label{sec:parrondoquantum}
\subsection{Defining the combined game}
As a reward for our efforts in part \textbf{I} of the dissertation and in the preceding section, we can now ignore the complicated Markov-quantum model and instead utilize the far simpler Markov-Bayesian-quantum model. Furthermore, since the latter model uses maps that live on a convex space, it is possible to utilize coin flips to combine two games instead of the recourse to more complicated alternating rules for rounds previously used by~\cite{flitney}~\cite{meyer}. This combined game has graphical model (note it is the same as (\ref{fig:combinedhiddengame})):
\begin{align}\label{fig:combinedquantumopen}
\setlength{\unitlength}{.8 in}
\begin{picture}(5.5,1.2)
\color{blue}
\put(.1,.1){\oval(.2,.2)[r]}
\put(0,.2){\line(1,0){.1}}
\put(0,0){\line(1,0){.1}}
\put(0,0){\line(0,1){.2}}
\put(1,.1){\circle{.2}}
\put(2,.1){\circle{.2}}
\put(3.5,.1){\circle{.2}}
\put(4.5,.1){\circle{.2}}
\put(5.5,.1){\oval(.2,.2)[l]}
\put(5.5,.2){\line(1,0){.1}}
\put(5.5,0){\line(1,0){.1}}
\put(5.6,0){\line(0,1){.2}}
\put(.2,.1){\vector(1,0){.7}}
\put(1.09,.1){\vector(1,0){.8}}
\put(2.09,.1){\line(1,0){.5}}
\put(2.89,.1){\vector(1,0){.5}}
\put(2.7,.05){$\cdots$}
\put(3.59,.1){\vector(1,0){.8}}
\put(4.59,.1){\vector(1,0){.8}}
\put(.89,.1){\line(0,1){.1}}
\put(1.89,.1){\line(0,1){.1}}
\put(3.39,.1){\line(0,1){.1}}
\put(4.39,.1){\line(0,1){.1}}
\color{black}
\put(1,.3){\circle{.2}}
\put(2,.3){\circle{.2}}
\put(3.5,.3){\circle{.2}}
\put(4.5,.3){\circle{.2}}
\put(1,.45){1}
\put(2,.45){2}
\put(3.5,.45){$ n-1 $}
\put(4.5,.45){\textit{n}}
\put(4.4,.3){\line(1,0){.19}}
\put(4.5,.209){\line(0,1){.185}}
\put(.89,.2){\line(0,1){.1}}
\put(1.89,.2){\line(0,1){.1}}
\put(3.39,.2){\line(0,1){.1}}
\put(4.39,.2){\line(0,1){.1}}
\put(.75,.8){\circle{.2}}
\put(1.75,.8){\circle{.2}}
\put(3.25,.8){\circle{.2}}
\put(4.25,.8){\circle{.2}}
\put(.78,.72){\vector(1,-4){.11}}
\put(1.78,.72){\vector(1,-4){.11}}
\put(3.28,.72){\vector(1,-4){.11}}
\put(4.28,.72){\vector(1,-4){.11}}
\put(.3,1){\{heads,tails\}}
\put(1.5,1){\{heads,tails\}}
\put(2.8,1){\{heads,tails\}}
\put(4,1){\{heads,tails\}}
\end{picture}
\end{align}
Again, let $ \gamma $ be the previously given probability measure for the coin of \textit{p} for heads and $ 1-p $ for tails, and, for simplicity of notation, identify $ \gamma $ with its Radon-Nikod\'{y}m derivative with respect to the counting measure. For the combined game, the map for each round is
\begin{equation}
M(\rho\otimes \gamma)=p\,L\rho+(1-p)L'\rho=L''\rho
\end{equation}  
for $ L''=p\,L+(1-p)L' $. Let $ N',N''\in\mathcal{B}\left(\mathcal{D}(\mathsf{H})\right) $ be defined using $ L',L''$ as \textit{N} was following (\ref{eq:probwinningquantum}),as $ N'=  S_{\mathcal{R}}\circ L' $ and  $ N''=  S_{\mathcal{R}}\circ L'' $. Then the marginal probability for the observation to be in \textit{A} for the $ n $th round (so Alice wins) is (compare to (\ref{eq:jointcombinedhiddenclassical}))
\begin{align}
P_{A,n}^{\text{comb}}&=\text{tr }S_{A}\circ M\left(\cdots\left(S_{\mathcal{R}}\circ M\left(\left(S_{\mathcal{R}}\circ M\rho_{0}\right)\otimes\gamma\right)\right)\otimes\gamma\cdots\right) d\mu\\&=\text{tr }S_{A}\circ L''\circ \underbrace{N''\circ\cdots\circ N''}_{n-1}\rho_{0} \nonumber
\end{align}
Because of the definition of the game, it is possible to reduce to the case where $ \mathcal{E}=\lbrace\varnothing, A,\tilde{A},\mathcal{X}\rbrace $.
\subsection{Bounds on the paradox for the quantum game}
Since it is possible to embed a classical hidden system within a quantum one (see \S\ref{sec:embedclassical}), one may expect the paradox to be present to an equal or greater degree for these quantum games. This is indeed the case, as is seen by comparing the statements of theorems \textbf{7.3.3} and \textbf{7.3.4} with the following theorem \textbf{7.5.3} and claim \textbf{7.5.5}. By analogy to definition \textbf{7.2.1}, we have:
\paragraph*{Definition 7.5.1} A linear map \textit{L} from $ \mathcal{D}(\mathsf{H})^{+} $ to  $ \mathcal{D}(\mathsf{H})^{+} $ has the \textit{quantum-Perron-Frobenius property}, $ \mathcal{QPF}(\mathsf{H}) $, if there is a density matrix $ \rho $, termed the \textit{quantum-Perron-Frobenius eigenvector}, such that the sequence $ \langle L^{j}\rho_{0}\rangle $ converges in total-variation norm to $ \rho $ regardless of the initial unit-norm density matrix $ \rho_{0} $.
\medskip\\
Restrict the space of pince-nez maps $ L,L' $ to those where $ N$ ,$N'$, and their convex combination, $ pN+(1-p)N' $, are all in $\mathcal{QPF}(\mathsf{H}) $. Then, once again, let $ P_{A}$, $ P'_{A} $, and $ P_{A}^{\text{comb}} $ be the limits as $ n\to \infty $ of $ P_{A,n} $, $ P'_{A,n}$ and $ P_{A,n}^{\text{comb}} $ respectively. 
\paragraph*{Definition 7.5.2} The \textit{quantum allowed region}, denoted $ \mathcal{Q}(A,\mathcal{X},\mathcal{E},\mathsf{H},p) $, is the set of all $\left(P_{A},P'_{A},P_{A}^{\text{comb}}\right)\in[0,1]^{\times 3} $ that occur, for fixed \textit{A}, $ \mathcal{X}$, $ \mathcal{E}$, \textsf{H},  and $ p $, over all allowed pince-nez maps \textit{L} and \textit{L}$ ' $. 
\medskip\\
As in the classical case, the existence of the paradox is then determined by the intersection of $ \mathcal{Q} $ with the cube $ \left(\frac{1}{2},1\right]\times\left(\frac{1}{2},1\right]\times\left[0,\frac{1}{2}\right) $. For $ p=1 $, $ P_{A}^{\text{comb}}=P_{A} $ and for $ p=0 $, $ P_{A}^{\text{comb}}=P'_{A} $; clearly no paradox is possible. We have the following theorem and claims for $ p\in(0,1) $, which indicate that, once again, there are basically only two possibilities, depending on whether we have $ \dim\mathsf{H}=2 $ or $ \dim\mathsf{H}>2  $.
\paragraph*{Theorem 7.5.3} For $ p\in (0,1) $, if $ \dim\mathsf{H}> 2 $, then $ \mathcal{Q}\supset(0,1)^{\times 3} $.
\paragraph*{Proof} Pick any $ \varepsilon>0 $ Let $ \mathsf{H}_{1},\mathsf{H}_{2},\mathsf{H}_{3} $ be three non-trivial subspaces of $ \mathsf{H} $ such that $ \mathsf{H}= \mathsf{H}_{1}\oplus\mathsf{H}_{2}\oplus\mathsf{H}_{3} $. Choose any density matrices $ \nu_{1}\in\mathcal{D}(\mathsf{H}_{1})^{+}$, $ \nu_{2}\in\mathcal{D}(\mathsf{H}_{2})^{+}$, $ \nu_{3}\in\mathcal{D}(\mathsf{H}_{3})^{+}$ with unit trace. Let $ \kappa:\mathcal{D}(\mathsf{H})^{+}\to\mathbb{R}^{3} $ be the map
\begin{equation}
\kappa(\rho)=\left[\begin{array}{c}\text{tr }\rho\vert_{\mathsf{H}_{1}}\\\text{tr }\rho\vert_{\mathsf{H}_{2}}\\\text{tr }\rho\vert_{\mathsf{H}_{3}}\end{array} \right]
\end{equation}
and define the pince-nez maps \textit{L} and $L' $ by
\begin{align}
L\rho&=1_{A}\otimes\left[\begin{array}{ccc}\nu_{1}&0&0\end{array}\right]\mathbf{T}\kappa(\rho)+1_{\tilde{A}}\otimes\left[\begin{array}{ccc}0&\nu_{2}&\nu_{3}\end{array}\right]\mathbf{T}\kappa(\rho)\\L'\rho&=1_{A}\otimes\left[\begin{array}{ccc}\nu_{1}&0&0\end{array}\right]\mathbf{T}'\kappa(\rho)+1_{\tilde{A}}\otimes\left[\begin{array}{ccc}0&\nu_{2}&\nu_{3}\end{array}\right]\mathbf{T}'\kappa(\rho)\nonumber
\end{align}
for $ \mathbf{T},\mathbf{T}' $ as in theorem \textbf{7.2.3}. Because of the properties of $ \nu_{1} $, $ \nu_{2} $, $ \nu_{3} $, and $ \kappa $, the required calculation reduces to matrix products, which then proceeds as in the proof for theorem \textbf{7.3.3}. $ \square $
\medskip\\

Employing a similar construction, for $ \dim \mathsf{H}=2 $ we have $ \mathcal{Q}(p)\supset\mathcal{CH}(p) $. We have the following two claims, backed by extensive numerical calculation:
\paragraph{Claim 7.5.4} For any fixed $ p,P_{A},P'_{A}\in(0,1) $, the minimum and maximum values of $ P_{A}^{\text{comb}} $ are achieved for pince-nez maps \textit{L} and $ L' $ each of the form $ \rho\to 1_{A}\otimes J\rho J^{*}+ 1_{\tilde{A}}\otimes K\rho K^{*}$.
\paragraph{Claim 7.5.5} For any fixed $ p,P_{A},P'_{A}\in(0,1) $, the minimum and maximum values of $ P_{A}^{\text{comb}} $ lie outside the bounds given in theorem \textbf{7.3.3}.
\medskip\\
Assuming the validity of the first claim, the extremizing maps can be expressed as 
\begin{align}
L\rho&=1_{A}\otimes\left[\begin{array}{cc}u_{1}&v_{1}\\u_{2}&v_{2}\end{array}\right]\rho\left[\begin{array}{cc}\overline{u_{1}}&\overline{u_{2}}\\\overline{v_{1}}&\overline{v_{2}}\end{array}\right]+1_{\tilde{A}}\otimes\left[\begin{array}{cc}u_{3}&v_{3}\\u_{4}&v_{4}\end{array}\right]\rho\left[\begin{array}{cc}\overline{u_{3}}&\overline{u_{4}}\\\overline{v_{3}}&\overline{v_{4}}\end{array}\right]\\L'\rho&=1_{A}\otimes\left[\begin{array}{cc}u'_{1}&v'_{1}\\u'_{2}&v'_{2}\end{array}\right]\rho\left[\begin{array}{cc}\overline{u'_{1}}&\overline{u'_{2}}\\\overline{v'_{1}}&\overline{v'_{2}}\end{array}\right]+1_{\tilde{A}}\otimes\left[\begin{array}{cc}u'_{3}&v'_{3}\\u'_{4}&v'_{4}\end{array}\right]\rho\left[\begin{array}{cc}\overline{u'_{3}}&\overline{u'_{4}}\\\overline{v'_{3}}&\overline{v'_{4}}\end{array}\right]\nonumber
\end{align}
for $ \Vert\vec{u}\Vert^{2}= \Vert\vec{v}\Vert^{2}=1 $, $ \vec{u}\perp\vec{v} $ except for points excluded by the requirement of the quantum Perron-Frobenius property. We are then faced by the following optimization problem, which may be treated numerically:
\begin{align}\label{eq:quantumextremize}
\text{constraints: }&\vec{w}\mathbf{M}^{-1}\left[\begin{array}{c}0\\0\\0\\1 \end{array}\right] =P_{A},\vec{w}'{\mathbf{M}'}^{-1}\left[\begin{array}{c}0\\0\\0\\1 \end{array}\right]=P'_{A}\\\text{extremize: }&P^{\text{comb}}_{A}=\left(p\vec{w}+(1-p)\vec{w}'\right)\left(p\mathbf{M}+(1-p)\mathbf{M}'\right)^{-1}\left[\begin{array}{c}0\\0\\0\\1 \end{array}\right]\nonumber
\end{align} 
for
\begin{align}
&\vec{w}=\left[\begin{array}{cccc}\vert u_{1} \vert^{2}+\vert u_{2} \vert^{2}&\hspace{.1 in}\overline{u_{1}}v_{1}+\overline{u_{2}}v_{2}&\hspace{.1 in} u_{1}\overline{v_{1}}+u_{2}\overline{v_{2}}&\hspace{.1 in}\vert v_{1} \vert^{2}+\vert v_{2} \vert^{2}\end{array} \right]\\&\vec{w}'=\left[\begin{array}{cccc}\vert u'_{1} \vert^{2}+\vert u'_{2} \vert^{2}&\hspace{.1 in}\overline{u'_{1}}v'_{1}+\overline{u'_{2}}v'_{2}&\hspace{.1 in} u'_{1}\overline{v'_{1}}+u'_{2}\overline{v'_{2}}&\hspace{.1 in}\vert v'_{1} \vert^{2}+\vert v'_{2} \vert^{2}\end{array} \right]\nonumber\\
&\mathbf{M}=\left[\begin{array}{cccc}\vert u_{1} \vert^{2}+\vert u_{3} \vert^{2}-1&\hspace{.1 in}\overline{u_{1}}v_{1}+\overline{u_{3}}v_{3}&\hspace{.1 in}\overline{v_{1}} u_{1}+\overline{v_{3}} u_{3}&\hspace{.1 in}\vert v_{1} \vert^{2}+\vert v_{3} \vert^{2}\\\overline{u_{1}}u_{2}+\overline{u_{3}}u_{4}&\hspace{.1 in}\overline{u_{1}}v_{2}+\overline{u_{3}}v_{4}-1&\hspace{.1 in}\overline{v_{1}} u_{2}+\overline{v_{3}} u_{4}&\hspace{.1 in}\overline{v_{1}} v_{2}+\overline{v_{3}} v_{4}\\\overline{u_{2}} u_{1}+\overline{u_{4}} u_{3}&\hspace{.1 in} \overline{u_{2}} v_{1}+\overline{u_{4}} v_{3}&\hspace{.1 in}\overline{v_{2}}u_{1}+\overline{v_{4}}u_{3}-1&\hspace{.1 in} \overline{v_{2}}v_{1}+\overline{v_{4}}v_{3}\\1&0&0&1\end{array}\right]\nonumber\\&{\mathbf{M}}'=\left[\begin{array}{cccc}\vert u'_{1} \vert^{2}+\vert u'_{3} \vert^{2}-1&\hspace{.1 in}\overline{u'_{1}}v'_{1}+\overline{u'_{3}}v'_{3}&\hspace{.1 in}\overline{v'_{1}} u'_{1}+\overline{v'_{3}} u'_{3}&\hspace{.1 in}\vert v'_{1} \vert^{2}+\vert v'_{3} \vert^{2}\\\overline{u'_{1}}u'_{2}+\overline{u'_{3}}u'_{4}&\hspace{.1 in}\overline{u'_{1}}v'_{2}+\overline{u'_{3}}v'_{4}-1&\hspace{.1 in}\overline{v'_{1}} u'_{2}+\overline{v'_{3}} u'_{4}&\hspace{.1 in}\overline{v'_{1}} v'_{2}+\overline{v_{3}} v'_{4}\\\overline{u'_{2}} u'_{1}+\overline{u'_{4}} u'_{3}&\hspace{.1 in} \overline{u'_{2}} v'_{1}+\overline{u'_{4}} v'_{3}&\hspace{.1 in}\overline{v'_{2}}u'_{1}+\overline{v'_{4}}u'_{3}-1&\hspace{.1 in} \overline{v'_{2}}v'_{1}+\overline{v'_{4}}v'_{3}\\1&0&0&1\end{array}\right]\nonumber
\end{align}
Graphs, for certain representative values of \textit{p}, of the minimum achievable $ P^{\text{comb}}_{A} $ given $ P_{A},P'_{A} $, are given in the following section.
\section{Summary of results}
In summary, for the considered classical game whose event space $ \mathcal{E} $ is effectively three or more states, the analogous classical hidden game whose $ \sigma $-algebra $ \mathcal{F} $ for its hidden set is effectively three or more states, and the analogous quantum game whose Hilbert space is three or more dimensions, we have proven there is no limitation on the probability for Alice to win the combined game, $ P^{\text{comb}}_{A} $, given her probabilities to win the individual games, $ P_{A}$ and $P'_{A} $. For the classical game with two-states, $ \mathcal{E}=\lbrace\varnothing, A,\tilde{A},\mathcal{O}\rbrace $, we have proven the paradox cannot occur. For the analogous classical hidden game with two-states, $ \mathcal{F}=\lbrace\varnothing, B,\tilde{B},\mathcal{H}\rbrace $, we have  
\begin{equation}
\min\lbrace pP_{A},(1-p)P'_{A}\rbrace<P^{\text{comb}}_{A}<\max\lbrace 1-p+pP_{A},p+(1-p)P'_{A}\rbrace
\end{equation}
where $ p\in(0,1) $ is the probability for the coin to land heads.

The following contour plots illustrate the lower bounds on $ P^{\text{comb}}_{A} $ for the two representative values of $ p=0.5 $ (the fair coin) and $ p=0.1 $. The paradox is displayed by minimum achievable values of $ P^{\text{comb}}_{A} $ being less than one-half in the region $ (P_{A},P'_{A})\in\left(\frac{1}{2},1\right]\times\left(\frac{1}{2},1\right] $. For comparison, plots of the minimum achieved $ P^{\text{comb}}_{A} $ for the analogous quantum game whose Hilbert space \textsf{H} has dimension two, which were numerically calculated from the optimization problem posed in (\ref{eq:quantumextremize}), are given as well.
\begin{figure}[p]
\setlength{\unitlength}{.85 in}
\begin{center}
\begin{picture}(5.5,4)
\put(.7,.1){\includegraphics[scale=.6]{parrondoparadoxminboundchp5.pdf}}
\put(2.7,.2){$ P_{A} $}
\put(.5,2.2){$ P'_{A} $}
\end{picture}
\end{center}
\caption{Minimum achievable values of $ P^{\text{comb}}_{A} $ for $ p=0.5 $ for the two-state, classical hidden game.}
\end{figure}
\begin{figure}[p]
\setlength{\unitlength}{.85 in}
\begin{center}
\begin{picture}(5.5,3.6)
\put(.7,.1){\includegraphics[scale=.6]{parrondoparadoxminboundchp1.pdf}}
\put(2.7,.2){$ P_{A} $}
\put(.5,2.2){$ P'_{A} $}
\end{picture}
\end{center}
\caption{Minimum achievable values of $ P^{\text{comb}}_{A} $ for $ p=0.1 $ for the two-state, classical hidden game.}
\end{figure}
\begin{figure}[p]
\setlength{\unitlength}{.85 in}
\begin{center}
\begin{picture}(5.5,3.9)
\put(.7,.1){\includegraphics[scale=.6]{parrondoparadoxminboundqp5.pdf}}
\put(2.7,.2){$ P_{A} $}
\put(.5,2.2){$ P'_{A} $}
\end{picture}
\end{center}
\caption{Minimum achievable values of $ P^{\text{comb}}_{A} $ for $ p=0.5 $ for the two-dimensional, quantum game.}
\end{figure}
\begin{figure}[p]
\setlength{\unitlength}{.85 in}
\begin{center}
\begin{picture}(5.5,3.6)
\put(.7,.1){\includegraphics[scale=.6]{parrondoparadoxminboundqp1.pdf}}
\put(2.7,.2){$ P_{A} $}
\put(.5,2.2){$ P'_{A} $}
\end{picture}
\end{center}
\caption{Minimum achievable values of $ P^{\text{comb}}_{A} $ for $ p=0.1 $ for the two-dimensional, quantum game.}
\end{figure}
